JADES: Balmer Decrement Measurements at redshifts 4 < z < 7

We present Balmer decrement H$\alpha$/ H$\beta$ measurements for a sample of 51 galaxies at redshifts z = 4-7 observed with the JWST/NIRSpec MSA, as part of the JADES survey. Leveraging 28-hour long exposures and the efficiency of the prism/clear configuration (but also using information from the medium-resolution gratings), we are able to probe directly the low-mass end of the galaxy population, reaching stellar masses Mstar as low as 10^7 Msun . We find that the correlation between Balmer decrement and Mstar is already established at these high redshifts, indicating a rapid build up of dust in moderately massive galaxies at such early epochs. The lowest-mass galaxies in our sample (Mstar = 1-3 x 10^7 Msun ) display a remarkably low Balmer decrement of 2.88 $\pm$ 0.08, consistent with case B, suggesting very little dust content. However, we warn that such a low observed Balmer decrement may also partly be a consequence of an intrinsically lower H$\alpha$/ H$\beta$, resulting from the extreme conditions of the ionized gas in these primeval and unevolved systems. We further compare the Balmer decrement to continuum-derived star-formation rates (SFR), finding tentative evidence of a correlation, which likely traces the underlying connection between SFR and mass of cold gas. However, we note that larger samples are required to distinguish between direct and primary correlations from indirect and secondary dependencies at such high redshifts.

==> additional <==
%  to add references on the fly

@BOOK{Osterbrock_2006,
       author = {{Osterbrock}, Donald E. and {Ferland}, Gary J.},
        title = "{Astrophysics of gaseous nebulae and active galactic nuclei}",
         year = 2006,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006agna.book.....O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{popping+2017,
       author = {{Popping}, Gerg{\"o} and {Somerville}, Rachel S. and {Galametz}, Maud},
        title = "{The dust content of galaxies from z = 0 to z = 9}",
      journal = {\mnras},
     keywords = {methods: numerical, dust, extinction, galaxies: evolution, galaxies: formation, galaxies: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = nov,
       volume = {471},
       number = {3},
        pages = {3152-3185},
          doi = {10.1093/mnras/stx1545},
archivePrefix = {arXiv},
       eprint = {1609.08622},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471.3152P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{charlot+2000,
       author = {{Charlot}, St{\'e}phane and {Fall}, S. Michael},
        title = "{A Simple Model for the Absorption of Starlight by Dust in Galaxies}",
      journal = {\apj},
     keywords = {ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Starburst, Infrared: Galaxies, Ultraviolet: Galaxies, Astrophysics},
         year = 2000,
        month = aug,
       volume = {539},
       number = {2},
        pages = {718-731},
          doi = {10.1086/309250},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003128},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..718C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...837L..21L,
       author = {{Laporte}, N. and {Ellis}, R.~S. and {Boone}, F. and {Bauer}, F.~E. and {Qu{\'e}nard}, D. and {Roberts-Borsani}, G.~W. and {Pell{\'o}}, R. and {P{\'e}rez-Fournon}, I. and {Streblyanska}, A.},
        title = "{Dust in the Reionization Era: ALMA Observations of a z = 8.38 Gravitationally Lensed Galaxy}",
      journal = {\apjl},
     keywords = {early universe, galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: star formation, submillimeter: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2017,
        month = mar,
       volume = {837},
       number = {2},
          eid = {L21},
        pages = {L21},
          doi = {10.3847/2041-8213/aa62aa},
archivePrefix = {arXiv},
       eprint = {1703.02039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837L..21L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022MNRAS.515.1751W,
       author = {{Witstok}, Joris and {Smit}, Renske and {Maiolino}, Roberto and {Kumari}, Nimisha and {Aravena}, Manuel and {Boogaard}, Leindert and {Bouwens}, Rychard and {Carniani}, Stefano and {Hodge}, Jacqueline A. and {Jones}, Gareth C. and {Stefanon}, Mauro and {van der Werf}, Paul and {Schouws}, Sander},
        title = "{Dual constraints with ALMA: new [O III] 88-{\ensuremath{\mu}}m and dust-continuum observations reveal the ISM conditions of luminous LBGs at z   7}",
      journal = {\mnras},
     keywords = {methods: observational, techniques: imaging spectroscopy, galaxies: high-redshift, dark ages, reionization, first stars, submillimetre: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = sep,
       volume = {515},
       number = {2},
        pages = {1751-1773},
          doi = {10.1093/mnras/stac1905},
archivePrefix = {arXiv},
       eprint = {2207.00022},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.515.1751W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...429..582C,
       author = {{Calzetti}, Daniela and {Kinney}, Anne L. and {Storchi-Bergmann}, Thaisa},
        title = "{Dust Extinction of the Stellar Continua in Starburst Galaxies: The Ultraviolet and Optical Extinction Law}",
      journal = {\apj},
     keywords = {Astronomical Models, Continuums, Distribution Functions, Interplanetary Dust, Interstellar Extinction, Metallicity, Spectra, Spectral Energy Distribution, Starburst Galaxies, Ultraviolet Spectra, Analytic Functions, Apertures, Average, Calibrating, Derivation, Extraction, Iue, Numerical Analysis, Optimization, Photometry, Astrophysics, GALAXIES: ISM, GALAXIES: PHOTOMETRY, GALAXIES: STARBURST, ISM: DUST, EXTINCTION, ULTRAVIOLET: GALAXIES},
         year = 1994,
        month = jul,
       volume = {429},
        pages = {582},
          doi = {10.1086/174346},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...429..582C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
